A fully implicit, asymptotic-preserving, semi-Lagrangian algorithm for the time dependent anisotropic heat transport equation

In this paper, we extend the operator-split asymptotic-preserving, semi-Lagrangian algorithm for time dependent anisotropic heat transport equation proposed in [Chac\'on et al., JCP, 272, 719-746, 2014] to use a fully implicit time integration with backward differentiation formulas. The proposed implicit method can deal with arbitrary heat-transport anisotropy ratios \chi_{\parallel}/\chi_{\perp}\ggg1 (with \chi_{\parallel}, \chi_{\perp} the parallel and perpendicular heat diffusivities, respectively) in complicated magnetic field topologies in an accurate and efficient manner. The implicit algorithm is second-order accurate temporally, has favorable positivity preservation properties, and demonstrates an accurate treatment at boundary layers (e.g., island separatrices), which was not ensured by the operator-split implementation. The condition number of the resulting algebraic system is independent of the anisotropy ratio, and is inverted with preconditioned GMRES. We propose a simple preconditioner that renders the linear system compact, resulting in mesh-independent convergence rates for topologically simple magnetic fields, and convergence rates scaling as \sim(N\Delta t)^{1/4} (with N the total mesh size and \Delta t the timestep) in topologically complex magnetic-field configurations. We demonstrate the accuracy and performance of the approach with test problems of varying complexity, including an analytically tractable boundary-layer problem in a straight magnetic field, and a topologically complex magnetic field featuring magnetic islands with extreme anisotropy ratios (\chi_{\parallel}/\chi_{\perp}=10^{10}).

==> prec.tex <==

\section{Preconditioning strategy}

\label{sec:prec} Equations (\ref{bdf1}) and (\ref{bdf2}) are implicit.
Thus, one needs to invert them at every time step. However, a matrix
representation for any given discretization of the operators $\mathcal{G}$
and $\mathcal{P}$ for arbitrary $\mathbf{B}$ is not known beforehand,
and would be extremely difficult to construct. Therefore, it is advantageous
to use robust matrix-free Krylov methods such as GMRES (generalized
minimal residual) \citep{saad1986gmres}. The convergence of Krylov
methods is sensitive to the spectrum of the corresponding operators,
and preconditioning is usually necessary to achieve competitive performance.
In this study, we first propose a preconditioner for the BDF1 temporal
scheme based on an asymptotic approximation to Eq. (\ref{bdf1}),
and later generalize it to BDF2.

Our goal is to find an effective preconditioner for the linear system
$\mathcal{L}=\mathbb{I}+\mathcal{P}\mathbb{B}$. We begin by introducing
new variables 
\begin{align}
\xi=\mathbb{B}T,\quad\xi_{N}=\mathcal{P}\xi,\quad\delta\xi=\xi-\xi_{N},
\end{align}
so after simple manipulations we find the following exact expressions:
\begin{align}
{\normalcolor \xi_{N}} & {\normalcolor =(\mathbb{I}+\mathbb{B})^{-1}(\mathbb{B}v-\delta\xi),}\label{eq:xi_n_exact}\\
{\normalcolor \delta\xi} & {\normalcolor =(\mathbb{I}-\mathcal{P})\mathbb{B}(v-\xi_{N}).}
\end{align}
Note that, in the limit of infinite anisotropy $\epsilon\rightarrow0$,
$\mathcal{P}$ turns into a projection operator onto the null space
of the $\nabla_{\parallel}^{2}$ operator, so $\mathcal{P}^{2}=\mathcal{P}$
and the new variables are projections onto and perpendicular to the
null space, respectively, namely: 
\begin{align}
\mathcal{P}\xi_{N}=\xi_{N},~~\mathcal{P}\delta\xi=0.
\end{align}

We formulate our preconditioner for Eq. (\ref{lin_system}) by making
the asymptotic approximation:
\begin{equation}
{\normalcolor \xi_{N}=(\mathbb{I}+\mathbb{B})^{-1}(\mathbb{B}v-\delta\xi)\approx\mathcal{P}\xi_{N}\approx\mathcal{P}(\mathbb{I}+\mathbb{B})^{-1}\mathbb{B}v,}\label{prec_aprox}
\end{equation}
so the preconditioner takes the final form: 
\begin{align}
{\normalcolor \xi_{N}} & {\normalcolor =\mathcal{P}(\mathbb{I}+\mathbb{B})^{-1}\mathbb{B}v,}\label{prec1}\\
{\normalcolor \delta\xi} & {\normalcolor =(\mathbb{I}-\mathcal{P})\mathbb{B}(v-\xi_{N}),}\label{prec2}\\
{\normalcolor T} & {\normalcolor =\mathbb{B}^{-1}(\xi_{N}+\delta\xi).}\label{prec3}
\end{align}
Note that, for high anisotropies, $\epsilon\ll1$, the approximation
(\ref{prec_aprox}) is exact when operators $\mathcal{P}$ and $\mathbb{B}$
commute (e.g., in straight magnetic fields). Indeed, 
\begin{align}
{\normalcolor \xi_{N}=\mathcal{P}\xi_{N}} & {\normalcolor =\mathcal{P}(\mathbb{I}+\mathbb{B})^{-1}\mathbb{B}v-\mathcal{P}(\mathbb{I}+\mathbb{B})^{-1}\delta\xi}\label{prec_err}\\
{\normalcolor } & {\normalcolor =\mathcal{P}(\mathbb{I}+\mathbb{B})^{-1}\mathbb{B}v-(\mathbb{I}+\mathbb{B})^{-1}\cancelto{0}{\mathcal{P}\delta\xi}}\\
{\normalcolor } & {\normalcolor =\mathcal{P}(\mathbb{I}+\mathbb{B})^{-1}\mathbb{B}v.}
\end{align}
Therefore, one can expect that preconditioner performance will be
exceptional in case of slightly curved magnetic fields and deteriorate
otherwise. The computational cost of the preconditioner is dominated
by the cost of the propagator $\mathcal{P}$. Therefore, a single
application of the preconditioner is about twice as expensive as the
evaluation of the linear residual of the main linear operator $\mathcal{L}$.

It is straightforward to extend the preconditioner to higher-order
BDF schemes. It is sufficient to notice that equation (\ref{lin_system})
stays the same for BDF2 (\ref{bdf2}) if one interprets the operator
$\mathcal{P}$ as a generalized projection operator. Therefore, to
generalize the preconditioner for the BDF2 scheme, one simply needs
to replace the definitions 
\begin{align}
{\normalcolor \mathcal{P}f} & {\normalcolor =\mathcal{P}\left(f,\mathbf{x},\frac{\Delta t}{\epsilon}\right),}\\
{\normalcolor \mathbb{B}f} & {\normalcolor =-\Delta t\nabla_{\perp}^{2}f,}
\end{align}
 with 
\begin{align}
{\normalcolor \mathcal{P}f} & {\normalcolor =2\mathcal{P}\left(f,\mathbf{x},\frac{\Delta t}{\epsilon}\right)-\mathcal{P}\left(f,\mathbf{x},\frac{2\Delta t}{\epsilon}\right),}\label{bdf2_P}\\
{\normalcolor \mathbb{B}f} & {\normalcolor =-\frac{2}{3}\Delta t\nabla_{\perp}^{2}f.}
\end{align}
Note that, in the limit $\epsilon\ll1$, the new operator (\ref{bdf2_P})
is still a projection operator, i.e., $\mathcal{P}^{2}=\mathcal{P}$.

\subsection{Preconditioned Krylov method convergence rate}

\label{sec:krylov_theory} The convergence of Krylov methods is sensitive
to the condition number of the linear operator. In this section, we
provide an estimate for the expected performance of the preconditioner
derived in Section~\ref{sec:prec}. The estimate for the number of
Krylov method iterations $N_{i}$ can be obtained from a condition
number $\kappa$ of the preconditioned linear system, i.e., 
\begin{align}
\mathcal{L}\mathcal{M}^{-1}\left(\mathcal{M}T\right)=v,
\end{align}
where $\mathcal{M}^{-1}$ is the preconditioner. Indeed, the number
of GMRES (or CG for SPD systems) iterations scales as $N_{i}\sim\sqrt{\kappa}$.
This can be shown readily from the usual CG convergence rate estimate
\citep{daniel1967conjugate}: 
\[
\left(\frac{\sqrt{\kappa}-1}{\sqrt{\kappa}+1}\right)^{N_{i}}=C_{tol}\Rightarrow N_{i}=\frac{\ln C_{tol}}{\ln\left(\frac{1-1/\sqrt{\kappa}}{1+1/\sqrt{\kappa}}\right)}\approx\frac{\ln C_{tol}}{\ln\left(1-2/\sqrt{\kappa}\right)}\approx\sqrt{\kappa}\ln\left(\frac{1}{\sqrt{C_{tol}}}\right),
\]
where $C_{tol}\ll1$ is a fixed constant determined by the specified
linear solver tolerance.

Following \ref{sec:prec_op}, we derive the expression for the preconditioned
operator in the limit of high anisotropy, when $\mathcal{P}$ acts
as a projection operator, i.e., $\mathcal{P}\approx\mathcal{P}^{2}$.
There results: 
\begin{align}
\mathcal{L}\mathcal{M}^{-1}\approx\mathbb{I}-\mathbb{B}^{-1}\left[\mathcal{P},\mathbb{B}\right](\mathbb{I}-\mathcal{P})\mathbb{B}(\mathbb{I}+\mathbb{B})^{-1}+O\left(\mathcal{P}^{2}-\mathcal{P}\right),\label{lm_prec}
\end{align}
where $[f,g]=fg-gf$ is the commutator operator. One can immediately
see that the leading source of error in the preconditioner (\ref{prec1})-(\ref{prec3})
is from the $\left[\mathcal{P},\mathbb{B}\right]$ term in (\ref{lm_prec}),
which is finite in the presence magnetic field curvature. Indeed,
if the magnetic field is straight, operators $\mathcal{P}$ and $\mathbb{B}$
commute and the term $\left[\mathcal{P},\mathbb{B}\right]$ vanishes
making the preconditioner ideal for high anisotropies. In the limit
of small curvature, the Fourier spectrum of the commutator can be
estimated as (see \ref{sec:curv_spec}) 
\begin{align}
\left[\mathcal{P},\mathbb{B}\right]e^{i\mathbf{x}\cdot\mathbf{k}}\sim\Delta tk^{2}e^{i\mathbf{x}\cdot\mathbf{k}}\sim\beta e^{i\mathbf{x}\cdot\mathbf{k}},\label{fop:c}
\end{align}
making the spectrum of $\mathcal{L}\mathcal{M}^{-1}$ bounded {[}using
(\ref{fop:p}) and (\ref{fop:c}){]}, since: 
\begin{align}
\rho\left(\mathcal{L}\mathcal{M}^{-1}\right)\sim1+\frac{\alpha\beta}{(1+\alpha)(1+\beta)}\sim1,
\end{align}
where we used 
\begin{align}
\rho\left(\mathbb{B}\right) & =\beta,\\
\rho\left(\mathbb{I}-\mathcal{P}\right) & =1-\frac{1-e^{-\alpha}}{\alpha}\sim\frac{\alpha}{1+\alpha},
\end{align}
and the last approximation is a conservative bound of the spectrum
of $\left(\mathbb{I}-\mathcal{P}\right)$ %\footnote{
%$$
%1 - \frac{1-e^{-\alpha}}{\alpha} = \left\{\begin{matrix}
%\alpha/2, & \alpha \ll 1, \\ 
%1 - 1/\alpha + e^{-\alpha}/\alpha, & \alpha \gg 1. 
%\end{matrix}\right.
%\quad
%\frac{\alpha}{1+\alpha} = \left\{\begin{matrix}
%\alpha, & \alpha \ll 1, \\ 
%1 - 1/\alpha, & \alpha \gg 1. 
%\end{matrix}\right.
%$$%
%}
for all practical values of $\alpha$, i.e., for null space $\alpha=0$
and off null space $\alpha\gg1$.

Unfortunately, it is quite difficult to estimate the spectrum of $[\mathcal{P},\mathbb{B}]$
for arbitrary magnetic field configurations. However, we conjecture
(and verify numerically later in this study) that for large enough
curvatures, the spectrum is modified by higher order $\beta$ terms
\begin{align}
\rho\left(\left[\mathcal{P},\mathbb{B}\right]\right)\sim0+\beta+C\beta^{2},
\end{align}
for some coefficient $C$. This leads to the following spectrum estimate
of the preconditioned operator for $\alpha\gg1$: 
\begin{align}
\rho\left(\mathcal{L}\mathcal{M}^{-1}\right)\sim1+\frac{\alpha\beta(1+C\beta)}{(1+\alpha)(1+\beta)}\sim1+C\beta,\label{eq:pc_cond_number}
\end{align}
which leads to the following condition number estimate of the preconditioned
system, $\mathcal{L}\mathcal{M}^{-1}$ (and corresponding GMRES iteration
count estimate): 
\begin{align}
\kappa\sim\beta\sim\frac{\Delta t}{\Delta},\quad\Rightarrow N_{i}\sim\frac{\sqrt{\Delta t}}{\Delta}\sim\sqrt{N\Delta t}.\label{krylov_pred}
\end{align}
Here, $\Delta$ is the characteristic cell size of the computational
grid, and $N\sim\Delta^{-2}$ is the total number of mesh points in
two dimensions.

